4D Gaussian Splatting for Real-Time Dynamic Scene Rendering

Representing and rendering dynamic scenes has been an important but challenging task. Especially, to accurately model complex motions, high efficiency is usually hard to guarantee. To achieve real-time dynamic scene rendering while also enjoying high training and storage efficiency, we propose 4D Gaussian Splatting (4D-GS) as a holistic representation for dynamic scenes rather than applying 3D-GS for each individual frame. In 4D-GS, a novel explicit representation containing both 3D Gaussians and 4D neural voxels is proposed. A decomposed neural voxel encoding algorithm inspired by HexPlane is proposed to efficiently build Gaussian features from 4D neural voxels and then a lightweight MLP is applied to predict Gaussian deformations at novel timestamps. Our 4D-GS method achieves real-time rendering under high resolutions, 82 FPS at an 800$\times$800 resolution on an RTX 3090 GPU while maintaining comparable or better quality than previous state-of-the-art methods. More demos and code are available at https://guanjunwu.github.io/4dgs/.

==> final_sup.tex <==

\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{fig/no_dx_vis.pdf}
   \caption{Visualization of ablation study about $\phi_x$.}
    \label{fig:no_dx_vis}
\end{figure}

\begin{figure*}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/editing_supp.pdf}
   \caption{More visualization of composition in 4D Gaussians. (a) Composition with Punch and Standup. (b) Composition with Lego and Trex. (c) Composition with Hellwarrior and Mutant. (d) Composition with Bouncingballs and Jumpingjacks.}
    \label{fig:editing_supp}
\end{figure*}
\begin{figure}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/ab_dshs.pdf}
   \caption{Visualization of ablation study in $\phi_{\mathcal{C}}$ and $\phi_{\mathcal{\alpha}}$ comparing with TiNeuVox~\cite{tineuvox}.}
    \label{fig:ab_dshs}
\end{figure}
\begin{figure*}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/grid_features2.pdf}
   \caption{More visualization of the HexPlane voxel grids $R(i,j)$ in bouncing balls. (a)-(c), (e)-(f) stand for visualization of $R_1(i,j)$, where grids resolution equals to 64$\times$64.}
    \label{fig:grid_feature_vis_supp}
\end{figure*}



\begin{figure}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/dycheck.pdf}
   \caption{Novel view rendering results in the iPhone datasets~\cite{dycheck}.}
    \label{fig:dycheck_supp}
\end{figure}

\begin{figure}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/sports.pdf}
   \caption{Rendering results on sports dataset~\cite{joo2015panopticstudio} also used in Dynamic3DGS~\cite{dynamic3dgs}.}
    \label{fig:sports_supp}
\end{figure}

\begin{figure}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/failurecases.pdf}
   \caption{Failure cases of modeling large motions and dramatic scene changes. (a) The sudden motion of the broom makes optimization harder. (b) Teapots have large motion and a hand is entering/leaving the scene.}
    \label{fig:failurecases}
\end{figure}


\begin{table*}	
\centering  
% \fontsize{6.5}{8}\selectfont  
\begin{threeparttable}  
\caption{Perscene results of HyperNeRF's vrig datasets~\cite{park2021hypernerf} by different models.}  
\label{tab:hypernerf_comparison}  
\begin{tabular}{l|cc|cc|cc|cc}  
\toprule  
\multirow{2}{*}{Method}&  
\multicolumn{2}{c}{3D Printer}&\multicolumn{2}{c}{Chicken}&\multicolumn{2}{c}{Broom}&\multicolumn{2}{c}{Banana}\cr  
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
&PSNR&MS-SSIM&PSNR&MS-SSIM&PSNR&MS-SSIM&PSNR&MS-SSIM\cr  
\midrule  
Nerfies~\cite{park2021nerfies}&20.6&0.83&26.7&0.94&19.2&0.56&22.4&0.87\cr  HyperNeRF~\cite{park2021hypernerf}&20.0&0.59&26.9&0.94&19.3&0.59&23.3&0.90\cr  
TiNeuVox-B~\cite{tineuvox}&\cellcolor{pink}22.8&\cellcolor{pink}0.84&\cellcolor{yellow}28.3&\cellcolor{pink}0.95&21.5&0.69&24.4\cellcolor{yellow}&\cellcolor{yellow}0.87\cr  
FFDNeRF~\cite{guo2023forwardflowfornvs}&\cellcolor{yellow}22.8&\cellcolor{yellow}0.84&28.0&\cellcolor{yellow}0.94&21.9\cellcolor{yellow}&0.71\cellcolor{pink}&24.3&0.86\cr
3D-GS~\cite{3dgs}&18.3&0.60&19.7&0.70&20.6&0.63&20.4&0.80\cr
Ours&22.1&0.81&\cellcolor{pink}28.7&0.93&\cellcolor{pink}22.0&0.70\cellcolor{yellow}&\cellcolor{pink}28.0&\cellcolor{pink}0.94\cr
\bottomrule  
\end{tabular}  
\end{threeparttable}  
\end{table*}  


\begin{table*}
\centering  
% \fontsize{6.5}{8}\selectfont  
\begin{threeparttable}  
\caption{Per-scene results of DyNeRF's~\cite{li2022neural} datasets.}  
\label{tab:dynerf_comparison}  
\begin{tabular}{l|cc|cc|cc}  
    \toprule  
    \multirow{2}{*}{Method}&  
    \multicolumn{2}{c}{Cut Beef}&\multicolumn{2}{c}{Cook Spinach}&\multicolumn{2}{c}{Sear Steak}\cr  
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    &PSNR&SSIM&PSNR&SSIM&PSNR&SSIM\cr  
    \midrule  
    NeRFPlayer~\cite{song2023nerfplayer}&31.83&0.928&32.06&0.930&32.31&0.940\cr
    HexPlane~\cite{hexplane}&\cellcolor{yellow}32.71&\cellcolor{pink}0.985&31.86&\cellcolor{pink}0.983&32.09&0.986\cr
    KPlanes~\cite{kplanes}&31.82&0.966&\cellcolor{pink}32.60&\cellcolor{yellow}0.966&\cellcolor{pink}32.52&\cellcolor{pink}0.974\cr
    MixVoxels~\cite{wang2023mixedvoxels}&31.30&0.965&31.65&0.965&31.43&\cellcolor{yellow}0.971\cr
    Ours&\cellcolor{pink}32.90&0.957&\cellcolor{yellow}32.46&0.949&\cellcolor{yellow}32.49&0.957\cr
\toprule  
    \multirow{2}{*}{Method}&  
    \multicolumn{2}{c}{Flame Steak}&\multicolumn{2}{c}{Flame Salmon}&\multicolumn{2}{c}{Coffee Martini}\cr  
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    &PSNR&SSIM&PSNR&SSIM&PSNR&SSIM\cr  
    \midrule
    NeRFPlayer~\cite{song2023nerfplayer}&27.36&0.867&26.14&0.849&\cellcolor{pink}32.05&\cellcolor{pink}0.938\cr
    HexPlane~\cite{hexplane}&31.92&\cellcolor{pink}0.988&\cellcolor{yellow}29.26&\cellcolor{pink}0.980&-&-\cr
    KPlanes~\cite{kplanes}&32.39&0.970&\cellcolor{pink}30.44&\cellcolor{yellow}0.953&29.99\cellcolor{yellow}&\cellcolor{yellow}0.953\cr
    MixVoxels~\cite{wang2023mixedvoxels}&31.21&\cellcolor{yellow}0.970&29.92&0.945&29.36&0.946\cr
    Ours&\cellcolor{pink}32.51&0.954&29.20&0.917&27.34&0.905\cr
    \bottomrule  
\end{tabular}  
\end{threeparttable}  
\end{table*}  

\begin{table*}
\centering  
\scalebox{0.9}{

% \fontsize{6.5}{8}\selectfont  
\begin{threeparttable}  
\caption{Per-scene results of synthesis datasets.}  
\label{tab:dnerf_comparison}  
\begin{tabular}{l|ccc|ccc|ccc|ccc}  
    \toprule  
    \multirow{2}{*}{Method}&  
    \multicolumn{3}{c}{Bouncing Balls}&\multicolumn{3}{c}{Hellwarrior}&\multicolumn{3}{c}{Hook}&\multicolumn{3}{c}{Jumpingjacks}\cr  
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
    &PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS\cr  
    \midrule  
    3D-GS~\cite{3dgs}&23.20&0.9591&0.0600&24.53&0.9336&0.0580\cellcolor{yellow}&21.71 & 0.8876& 0.1034& 23.20&0.9591 &0.0600\cr  
    K-Planes\cite{kplanes}&40.05&\cellcolor{yellow}0.9934&0.0322\cellcolor{yellow}&24.58&0.9520&0.0824&28.12&0.9489&0.0662&31.11&0.9708&0.0468\cr  
    HexPlane\cite{hexplane}&39.86&0.9915&0.0323&24.55&0.9443&0.0732&28.63&0.9572\cellcolor{yellow}&0.0505\cellcolor{yellow}&31.31&0.9729&0.0398\cr  
    TiNeuVox\cite{tineuvox}&\cellcolor{yellow}40.23&0.9926&0.0416&\cellcolor{yellow}27.10&\cellcolor{yellow}0.9638&0.0768&28.63\cellcolor{yellow}&0.9433&0.0636&33.49\cellcolor{yellow}&0.9771\cellcolor{yellow}&0.0408\cellcolor{yellow}\cr  		Ours&\cellcolor{pink}40.62&\cellcolor{pink}0.9942&\cellcolor{pink}0.0155&\cellcolor{pink}28.71&\cellcolor{pink}0.9733&\cellcolor{pink}0.0369&\cellcolor{pink}32.73&\cellcolor{pink}0.9760&\cellcolor{pink}0.0272&\cellcolor{pink}35.42&\cellcolor{pink}0.9857&\cellcolor{pink}0.0128\cr  
\toprule  
\multirow{2}{*}{Method}&  
    \multicolumn{3}{c}{Lego}&\multicolumn{3}{c}{Mutant}&\multicolumn{3}{c}{ Standup}&\multicolumn{3}{c}{Trex}\cr  
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
    &PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS&PSNR&SSIM&LPIPS\cr  
    \midrule  
    3D-GS~\cite{3dgs}&23.06&0.9290&0.0642&20.64&0.9297&0.0828&21.91&0.9301&0.0785&21.93&0.9539&0.0487\cr  
    K-Planes~\cite{kplanes}&\cellcolor{pink}25.49&\cellcolor{pink}0.9483&\cellcolor{pink}0.0331&32.50&0.9713&0.0362&33.10&0.9793&0.0310&30.43&0.9737&0.0343\cr  
    HexPlane~\cite{hexplane}&\cellcolor{yellow}25.10&\cellcolor{yellow}0.9388&0.0437&33.67\cellcolor{yellow}&0.980\cellcolor{yellow}2&0.0261\cellcolor{yellow}&34.40&\cellcolor{yellow}0.9839&\cellcolor{yellow}0.0204&30.67&\cellcolor{yellow}0.9749&\cellcolor{yellow}0.0273\cr  
    TiNeuVox~\cite{tineuvox}&24.65&0.9063&0.0648&30.87&0.9607&0.0474&\cellcolor{yellow}34.61&0.9797&0.0326&\cellcolor{yellow}31.25&0.9666&0.0478\cr  
    Ours&25.03&0.9376&0.0382\cellcolor{yellow}&\cellcolor{pink}37.59&\cellcolor{pink}0.9880&\cellcolor{pink}0.0167&\cellcolor{pink}38.11&\cellcolor{pink}0.9898&\cellcolor{pink}0.0074&\cellcolor{pink}34.23&\cellcolor{pink}0.9850&\cellcolor{pink}0.0131\cr  
    % B&0.7667&0.7644&0.7646&0.6609&0.6687&0.6574\cr  
    % A&{\bf 0.8189}&{\bf 0.8139}&{\bf 0.8146}&{\bf 0.6971}&{\bf 0.6904}&{\bf 0.6935}\cr  
    \bottomrule  
\end{tabular}  
\end{threeparttable}  
}
\end{table*}  


\begin{table}
\centering  
% \fontsize{6.5}{8}\selectfont  
\caption{Ablation Study on $\phi_{\mathcal{C}}$ and $\phi_{\mathcal{\alpha}}$, comparing with TiNeuVox~\cite{tineuvox} in Americano of HyperNeRF~\cite{park2021hypernerf}'s dataset.}
\begin{threeparttable}  
\label{tab:ablation_dshsdo}  
\begin{tabular}{l|cc }  
\toprule  
\multirow{2}{*}{Method}&  
\multicolumn{2}{c}{Americano}\cr  
\cmidrule(lr){2-3}
&PSNR&MS-SSIM\cr  
\midrule  
TiNeuVox-B~\cite{tineuvox}&28.4&0.96\cr  
Ours w/ $\phi_{\mathcal{C}}$,$\phi_{\mathcal{\alpha}}$ &\cellcolor{pink}31.53&\cellcolor{pink}0.97\cr
Ours&\cellcolor{yellow}30.90&\cellcolor{yellow}0.96\cr
\bottomrule  

\end{tabular}  
\end{threeparttable}  
\label{table:ab_dshsdo}

\end{table}  
\appendix

\section{Appendix}

\subsection{Introduction}
In the supplementary material, we mainly introduce our hyperparameter settings of experiments in Sec.~\ref{Supsec:hyperparameters}. Then more ablation studies are conducted in Sec.~\ref{Supsec:ablationstudies}. Finally, we delve into the limitations of our proposed 4D-GS in Sec.~\ref{supsec:discussions}.


\subsection{Hyperparameter Settings}
\label{Supsec:hyperparameters}
Our hyperparameters mainly follow the settings of 3D-GS~\cite{3dgs}. The basic resolution of our multi-resolution HexPlane module $R(i,j)$ is set to 64, which is upsampled by 2 and 4. The learning rate is set as $1.6\times10^{-3}$, decayed to $1.6e-4$ at the end of training. The Gaussian deformation decoder is a tiny MLP with a learning rate of $1.6\times10^{-3}$ which decreases to $1.6\times10^{-3}$. The batch size in training is set to 1. The opacity reset operation in \cite{3dgs} is not used as it does not bring evident benefit in most of our tested scenes. Besides, we find that expanding the batch size will indeed contribute to rendering quality but the training cost increases accordingly.

Different datasets are constructed under different capturing settings. D-NeRF~\cite{pumarola2021dnerf} is a synthesis dataset in which each timestamp has only one single captured image following the monocular setting. This dataset has no background which is easy to train, and can reveal the upper bound of our proposed framework. We change the pruning interval to 8000 and only set a single upsampling rate of the multi-resolution HexPlane Module $R(i,j)$ as 2 because the structure information is relatively simple in this dataset. The training iteration is set to 20000 and we stop 3D Gaussians from growing at the iteration of 15000.

The DyNeRF dataset~\cite{li2022neural} includes 15 -- 20 fixed camera setups, so it's easy to get the sfm~\cite{schonberger2016structurefrommotion} point in the first frame, we utilize the dense point-cloud reconstruction and downsample it lower than 100k to avoid out of memory error. Thanks to the efficient design of our 4D Gaussian splatting framework and the tiny movement of all the scenes, only 14000 iterations are needed and we can get the high rendering quality images. 
% The visualization of our model is shown in Fig.~\ref{fig:dynerf_result_vis}.

HyperNeRF's dataset is captured with less than 2 cameras in feed-forward settings. We change the upsampling resolution up to $[2,4]$ and the hidden dim of the decoder into 256. Similar to other works~\cite{tineuvox,park2021hypernerf}, we found that Gaussian deformation fields always fall into the local minima that link the correlation of motion between cameras and objects even with static 3D Gaussian initialization. And we're going to reserve the splitting of the relationship in the future works. 
% The visualization of our model is shown in Fig.~\ref{fig:hypernerf_result_sup}.

\subsection{More Ablation Studies}
\label{Supsec:ablationstudies}
\paragraph{Position Deformation.} We find that removing the output of the position deformation head can also model the object motion. It is mainly because leaving some 3D Gaussians in the dynamic part, keeping them small in shape, and then scaling them up at a certain timestamp can also model the dynamic part. However, this approach can only model coarse object motion and lost potential for tracking. The visualization is shown in Fig.~\ref{fig:no_dx_vis}.
\paragraph{Editing with 4D Gaussians.}
We provide more visualization in editing with 4D Gaussians with Fig.~\ref{fig:editing_supp}.  This work only proposes a naive approach to transformation. It is worth noting that when applying the rotation of the scenes, 3D Gaussian's rotation quaternion $q$ and scaling coefficient $s$ need to be considered. Meanwhile, some interpolation methods should be applied to enlarge or reduce 4D Gaussians.
\paragraph{Color and Opacity's Deformation.}
When encountered with fluid or non-rigid motion, we adopt another two output MLP decoder $\phi_{\mathcal{C}}$, $\phi_\alpha$ to compute the deformation of 3D Gaussian's color and opacity $\Delta \mathcal{C} = \phi_{\mathcal{C}}(f_d)$, $\Delta \alpha = \phi_{\mathcal{\alpha}}(f_d)$. Tab.~\ref{table:ab_dshsdo} and Fig.~\ref{fig:ab_dshs} show the results in comparison with TiNeuVox~\cite{tineuvox}. However, it is worth noting that modeling Gaussian color and opacity change may cause irrational shape changes when rendering novel views. \ie the Gaussians on the surface should move with other Gaussians but stay in the place and the color is changed, making the tracking difficult to achieve.
\paragraph{Spatial-temporal Structure Encoder.}
We have explored why 4D-GS can achieve such a fast convergence speed and rendering quality. As shown in Fig.~\ref{fig:grid_feature_vis_supp}, we visualize the full features of $R_1$ in bouncingballs. It's explicit that in the $R_1(x,y)$ plane, the spatial structure of the scenes is encoded. Similarily, $R_1(x,z)$ and $R_1(y,z)$ also show different view structure features. Meanwhile, temporal voxel grids $R_1(x,t),R_1(y,t)$ and $R_1(z,t)$ also show the integrated motion of the scenes, where large motions always stand for explicit features. So, it seems that the proposed HexPlane module encodes the features of spatial and temporal information.


\subsection{More Discussions}
\label{supsec:discussions}
\paragraph{Monocular Dynamic Scene Reconstruction.}
In monocular settings, input data are sparse from both cameration pose and timestamp dimensions. This may cause the local minima of overfitting with training images in some complicated scenes. As shown in Fig.~\ref{fig:dycheck_supp}, though 4D-GS can render relatively high quality in the training set, the strong overfitting effects of the proposed model cause the failure of rendering novel views. To solve the problem, more priors such as depth supervision or optical flow may be needed.

\paragraph{Large Motion Modeling with Multi-Camera Settings.}
In the DyNeRF~\cite{li2022neural}'s dataset, all the motion parts of the scene are not very large and the multi-view camera setup also provides a dense sampling of the scene. That is the reason why 4D-GS can perform a relatively high rendering quality. However, in large motion such as sports datasets~\cite{joo2015panopticstudio} used in~\cite{dynamic3dgs}, 4DGS cannot fit well within short times as shown in Fig.~\ref{fig:sports_supp}. Online training~\cite{dynamic3dgs,abou2022particlenerf} or using information from other views like~\cite{lin2023im4d,wang2021ibrnet} could be a better approach to solve the problem with multi-camera input.

\paragraph{Large Motion Modeling with Monocular Settings.}
4D-GS uses a deformation field network to model the motion of 3D Gaussians, which may fail in modeling large motions or dramatic scene changes. This phenomenon is also observed in previous NeRF-based methods~\cite{tineuvox,pumarola2021dnerf,park2021hypernerf,li2022neural}, producing blurring results. Fig.~\ref{fig:failurecases} shows some failed samples. Exploring more useful priors could be a promising future direction.

% also needs sufficient training strategies. In some cases such as large and sudden motion like broom or teapot in Fig.~\ref{fig:failurecases}, 4D-GS struggles to render time-aware sequential images, making novel views \textbf{splitting} instead of \textbf{blurring} previous NeRF-based methods~\cite{tineuvox,pumarola2021dnerf,park2021hypernerf,li2022neural}.

% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{main}
% }
% \end{document}




==> sec/0_abstract.tex <==
\begin{abstract}
% the importance of the problem
Representing and rendering dynamic scenes has been an important but challenging task. Especially, to accurately model complex motions, high efficiency is usually hard to guarantee. To achieve real-time dynamic scene rendering while also enjoying high training and storage efficiency, we propose 4D Gaussian Splatting (4D-GS) as a holistic representation for dynamic scenes rather than applying 3D-GS for each individual frame. In 4D-GS, a novel explicit representation containing both 3D Gaussians and 4D neural voxels is proposed. A decomposed neural voxel encoding algorithm inspired by HexPlane is proposed to efficiently build Gaussian features from 4D neural voxels and then a lightweight MLP is applied to predict Gaussian deformations at novel timestamps.
Our 4D-GS method achieves real-time rendering under high resolutions, 82 FPS at an 800$\times$800 resolution on an RTX 3090 GPU while maintaining comparable or better quality than previous state-of-the-art methods. More demos and code are available at \url{https://guanjunwu.github.io/4dgs/}. 
% We introduce 4D-GS for novel view synthesis in dynamic scenes by proposing a novel time-aware Gaussian splatting representation. Leveraging the combined strength of the HexPlane voxel deformation field and 3D-GS, the proposed 4D-GS method boasts a comparatively faster convergence speed and supports real-time rendering at 70 FPS in 800$\times$800 resolution on an RTX 3090 GPU. Experimental results validate that our approach achieves state-of-the-art performance on established benchmarks.
\end{abstract}

==> sec/1_intro.tex <==


\section{Introduction}
\label{sec:intro}
Novel view synthesis (NVS) stands as a critical task in the domain of 3D vision and plays a vital role in many applications, \eg VR, AR, and movie production. NVS aims at rendering images from any desired viewpoint or timestamp of a scene, usually requiring modeling the scene accurately from several 2D images. Dynamic scenes are quite common in real scenarios, rendering which is important but challenging as complex motions need to be modeled with both spatially and temporally sparse input.

NeRF~\cite{mildenhall2021nerf} has achieved great success in synthesizing novel view images by representing scenes with implicit functions. The volume rendering techniques~\cite{drebin1988volume} are introduced to connect 2D images and 3D scenes. However, the original NeRF method bears big training and rendering costs. Though some NeRF variants~\cite{dvgo,tineuvox,hexplane,kplanes,tensor4d,fridovich2022plenoxels,instantngp} reduce the training time from days to minutes, the rendering process still bears a non-negligible latency.

Recent 3D Gaussian Splatting (3D-GS)~\cite{3dgs} significantly boosts the rendering speed to a real-time level by representing the scene as 3D Gaussians. The cumbersome volume rendering in the original NeRF is replaced with efficient differentiable splatting~\cite{yifan2019differentiablesplatting}, which directly projects 3D Gaussian points onto the 2D plane. 3D-GS not only enjoys real-time rendering speed but also represents the scene more explicitly, making it easier to manipulate the scene representation. 

However, 3D-GS focuses on the static scenes. Extending it to dynamic scenes as a 4D representation is a reasonable, important but difficult topic. The key challenge lies in modeling complicated point motions from sparse input. 3D-GS holds a natural geometry prior by representing scenes with point-like Gaussians. One direct and effective extension approach is to construct 3D Gaussians at each timestamp~\cite{dynamic3dgs} but the storage/memory cost will multiply especially for long input sequences. Our goal is to construct a compact representation while maintaining both training and rendering efficiency, \ie 4D Gaussian Splatting (\textbf{4D-GS}). To this end, we propose to represent Gaussian motions and shape changes by an efficient Gaussian deformation field network, containing a temporal-spatial structure encoder and an extremely tiny multi-head Gaussian deformation decoder. Only one set of canonical 3D Gaussians is maintained. For each timestamp, the canonical 3D Gaussians will be transformed by the Gaussian deformation field into new positions with new shapes. The transformation process represents both the Gaussian motion and deformation. Note that different from modeling motions of each Gaussian separately~\cite{dynamic3dgs,4dgs-2}, the spatial-temporal structure encoder can connect different adjacent 3D Gaussians to predict more accurate motions and shape deformation. Then the deformed 3D Gaussians can be directly splatted for rendering the according-timestamp image. Our contributions can be summarized as follows.

\begin{itemize}
     \item An efficient 4D Gaussian splatting framework with an efficient Gaussian deformation field is proposed by modeling both Gaussian motion and Gaussian shape changes across time.
     \item A multi-resolution encoding method is proposed to connect the nearby 3D Gaussians and build rich 3D Gaussian features by an efficient spatial-temporal structure encoder. 
     \item 4D-GS achieves real-time rendering on dynamic scenes, up to 82 FPS at a resolution of 800$\times$800 for synthetic datasets and 30 FPS at a resolution of 1352$\times$1014 in real datasets, while maintaining comparable or superior performance than previous state-of-the-art (SOTA) methods and shows potential for editing and tracking in 4D scenes.
     % This performance surpasses that of other implementations.
\end{itemize}

==> sec/2.5_preliminary.tex <==
\section{Preliminary}
In this section, we simply review the representation and rendering process of 3D-GS~\cite{3dgs} in Sec.~\ref{subsec:3D Gaussian Splatting} and the formula of dynamic NeRFs in Sec.~\ref{subsec:Dynamic NeRFs with deformation Fields.}.

\subsection{3D Gaussian Splatting}
\label{subsec:3D Gaussian Splatting}
3D Gaussians~\cite{3dgs} is an explicit 3D scene representation in the form of point clouds. Each 3D Gaussian is characterized by a covariance matrix $\Sigma$ and a center point $\mathcal{X}$, which is referred to as the mean value of the Gaussian:
\begin{equation}
\label{formula:gaussian's formula}
    G(X)=e^{-\frac{1}{2}\mathcal{X}^T\Sigma^{-1}\mathcal{X}}.
\end{equation}
For differentiable optimization, the covariance matrix $\Sigma$ can be decomposed into a scaling matrix $\mathbf{S}$ and a rotation matrix $\mathbf{R}$:
\begin{equation}
\label{formula:covariance decomposition}
    \Sigma = \mathbf{R}\mathbf{S}\mathbf{S}^T\mathbf{R}^T.
\end{equation}
% the computation of gradient flow during training is depicted in~\cite{3dgs}.

When rendering novel views, differential splatting~\cite{yifan2019differentiablesplatting} is employed for the 3D Gaussians within the camera planes. As introduced by~\cite{zwicker2001surfacesplatting}, using a viewing transform matrix $W$ and the Jacobian matrix $J$ of the affine approximation of the projective transformation, the covariance matrix $\Sigma^{\prime}$ in camera coordinates can be computed as
\begin{equation}
    \Sigma^{\prime} = JW\Sigma W^TJ^T.
\end{equation}
In summary, each 3D Gaussian is characterized by the following attributes: position $\mathcal{X} \in \mathbb{R}^3$, color defined by spherical harmonic (SH) coefficients $\mathcal{C} \in \mathbb{R}^k$ (where $k$ represents nums of SH functions), opacity $\alpha \in \mathbb{R}$, rotation factor $r \in \mathbb{R}^4$, and scaling factor $s \in \mathbb{R}^3$.
Specifically, for each pixel, the color and opacity of all the Gaussians are computed using the Gaussian's representation Eq.~\ref{formula:gaussian's formula}. The blending of $N$ ordered points that overlap the pixel is given by the formula:
\begin{equation}
\label{formula: splatting&volume rendering}
    C = \sum_{i\in N}c_i \alpha_i \prod_{j=1}^{i-1} (1-\alpha_i).
\end{equation}
Here, $c_i$, $\alpha_i$ represents the density and color of this point computed by a 3D Gaussian $G$ with covariance $\Sigma$ multiplied by an optimizable per-point opacity and SH color coefficients.

\subsection{Dynamic NeRFs with Deformation Fields}
\label{subsec:Dynamic NeRFs with deformation Fields.}
All the dynamic NeRF algorithms can be formulated as:
\begin{equation}
    c,\sigma = \mathcal{M}(\mathbf{x},t),
\end{equation}
where $\mathcal{M}$ is a mapping that maps 6D space $(\mathbf{x},d,t)$ to 4D space $(c,\sigma)$. Dynamic NeRFs mainly follow two paths: canonical-mapping volume rendering~\cite{pumarola2021dnerf,park2021nerfies,park2021hypernerf,tineuvox,robustdynamicradiancefields} and time-aware volume rendering~\cite{Dynamicviewsynthesisfromdynamicmonocularvideo,li2022neural,hexplane,kplanes,tensor4d}. In this section, we mainly give a brief review of the former.

 As is shown in Fig.~\ref{fig: splatting-volume}~\textcolor{red}{(a)}, the canonical-mapping volume rendering transforms each sampled point into a canonical space by a deformation network $\phi_t:(\mathbf{x},t)\rightarrow \Delta \mathbf{x}$. Then a canonical network $\phi_x$ is introduced to regress volume density and view-dependent RGB color from each ray. The formula for rendering can be expressed as:
\begin{equation}
    c, \sigma = \text{NeRF}(\mathbf{x}+\Delta \mathbf{x}),
\end{equation}
where `NeRF' stands for vanilla NeRF pipeline.
% \paragraph{Time-aware Volume Rendering.} Fig.~\ref{fig: splatting-volume}~\textcolor{red}{(b)} illustrates the details of time-aware volume rendering. Though the rendering rays remain the same in 3D space, the temporal information is different, which means the sampled points are individual in the 4D space. Canonical network $\phi_x$ is introduced to combine the relationship between temporal and spatial features. 

However, our 4D Gaussian splatting framework presents a novel rendering technique. We transform 3D Gaussians using a Gaussian deformation field network $\mathcal{F}$ at the time $t$ directly and differential splatting~\cite{3dgs} is followed. 
% In most cases~\cite{pumarola2021dnerf,tineuvox,park2021hypernerf,dynamicnerf,park2021hypernerf}, positional encoding~\cite{vaswani2017attention} is used to expand information. 


% Approaches such as~\cite{kplanes,hexplane,tensor4d} provide effective dynamic scene representations that learn information from multi-view temporal image inputs and generate high-quality novel views. All of these approaches aim to regress color $c$ and density $\sigma$ given spatial point $x$ and time $t$ using a function $\mathbf{F}$:
% \begin{equation}
%     c, \sigma = \mathbf{F}(\mathcal{X},t).
% \end{equation}
% In most cases, $\mathbf{F}$ consists of a neural voxel module $\mathcal{F}$ and an MLP decoder $g$. During the forward pass, the point $x$ and time $t$ are fed into the voxel-plane module $\mathcal{F}$ to obtain voxel features $f_{voxel}$, and then the color $c$ and density $\sigma$ can be computed using the decoder $g$. Therefore, the forward process can be expressed as:

% \begin{align}
%       &  f_{voxel} = \mathcal{F}(X,t), \\
%   &  c, \sigma = g(f).
% \end{align}


==> sec/2_relatedworks.tex <==

\begin{figure}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/splatting_volume.pdf}
   \caption{Illustration of different dynamic scene rendering methods. (a) Points are sampled in the casted ray during volume rendering. The point deformation fields proposed in~\cite{pumarola2021dnerf, tineuvox} map the points into a canonical space. (b) Time-aware volume rendering computes the features of each point directly and does not change the rendering path. (c) The Gaussian deformation field converts original 3D Gaussians into another group of 3D Gaussians with a certain timestamp.}
   \label{fig: splatting-volume}
   \vspace{-10pt}
\end{figure}

\begin{figure*}[thbp]
   \centering
   \includegraphics[width=1.0\linewidth]{fig/pipeline.pdf}
   \caption{The overall pipeline of our model. Given a group of 3D Gaussians $\mathcal{G}$, we extract the center coordinate of each 3D Gaussian $\mathcal{X}$ and timestamp $t$ to compute the voxel feature by querying multi-resolution voxel planes. Then a tiny multi-head Gaussian deformation decoder is used to decode the feature and get the deformed 3D Gaussians $\mathcal{G}^\prime$ at timestamp $t$. The deformed Gaussians are then splatted to the rendered image.}
   \label{fig: pipeline}
   \vspace{-10pt}
\end{figure*}
\section{Related Works}
In this section, we simply review the difference of dynamic NeRFs in Sec.~\ref{subsec:dynamic novel view synthesis}, then discuss the point clouds-based neural rendering algorithm in Sec.~\ref{subsec:neural rendering with point clouds}.

\subsection{Neural Rendering}
\label{subsec:dynamic novel view synthesis}
Light fields can efficiently render novel views with dense image input. Mesh-based representations succeed in maintaining real-time rendering with modern rasterization pipelines. Voxel grids and multi-plane images also support gradient optimization. \cite{mildenhall2021nerf,barron2021mip,zhang2020nerf++} demonstrate that implicit radiance fields can effectively learn scene representations and synthesize high-quality novel views.~\cite{pumarola2021dnerf,park2021nerfies,park2021hypernerf} have challenged the static hypothesis, expanding the boundary of novel view synthesis for dynamic scenes. Additionally,~\cite{tineuvox} proposes to use an explicit voxel grid to model temporal information, accelerating the learning time for dynamic scenes to half an hour and applied in~\cite{gneuvox,robustdynamicradiancefields,guo2023forwardflowfornvs}. The proposed canonical mapping neural rendering methods are shown in Fig.~\ref{fig: splatting-volume} \textcolor{red} {(a)}. ~\cite{li2022neural,hexplane,kplanes,tensor4d,msth} represent further advancements in faster dynamic scene learning by adopting decomposed neural voxels. They treat sampled points in each timestamp individually as shown in Fig.~\ref{fig: splatting-volume} \textcolor{red} {(b)}.~\cite{wang2023neus2,gao2022mps,mlpmaps,xu2022multigeometric,lin2023im4d,wang2023mixedvoxels} are efficient methods to handle multi-view setups. The aforementioned methods though achieve fast training speed, real-time rendering for dynamic scenes is still challenging, especially for monocular input. Our method aims at constructing a highly efficient training and rendering pipeline in Fig.~\ref{fig: splatting-volume} \textcolor{red} {(c)}, while maintaining the quality, even for sparse inputs.
% While the methods mentioned above offer fast training speeds, the process of rendering an image still cannot achieve real-time performance. Meanwhile, Our proposed method is an efficient solution to achieve both high-quality novel view synthesis and extremely fast rendering speed.

% \paragraph{Accelerating Neural Rendering.}\label{subsec:Accelerating Dynamic NeRF's Rendering Speed}
% \cite{yu2021plenoctrees,hedman2021baking,reiser2021kilonerf,fridovich2022plenoxels,dvgo,instantngp} use explicit representations or the baking method to promote the training and rendering speed but mainly focus on the static scenes. Some works~\cite{mlpmaps, wang2022fourierplenoctrees,lin2023im4d} aim at accelerating the rendering on dynamic scenes but multi-view setups are needed. It becomes a growing demand to achieve general real-time rendering methods for dynamic scenes at sparse sequential camera setups. 3D Gaussian Splatting (3D-GS)~\cite{3dgs}, an effective scene representation and rendering method, has been developed that not only achieves fast convergence speeds but is also easily integrated into the graphics rendering pipeline, making real-time rendering of general scenes more accessible. Our method extends 3D-GS~\cite{3dgs} to 4D, named 4D-GS, achieving real-time rendering for general dynamic scenes that can be applied easily with both monocular and multi-view input.

\subsection{Neural Rendering with Point Clouds}\label{subsec:neural rendering with point clouds}
Effectively representing 3D scenes remains a challenging topic. The community has explored various neural representations~\cite{mildenhall2021nerf}, \eg meshes, point clouds~\cite{pointnerf}, and hybrid approaches. Point-cloud-based methods~\cite{qi2017pointnet,qi2017pointnet++,yu2018pu,liu2019meteornet} initially target at 3D segmentation and classification. A representative approach for rendering presented in~\cite{pointnerf, abou2022particlenerf} combines point cloud representations with volume rendering, achieving rapid convergence speed.~\cite{keselman2023flexibleTechniquesDifferentiableRendering,keselman2022approximatedifferentiablerenderingwithalgebraicsurfaces,ruckert2022adop} adopt differential point rendering technique for scene reconstructions. Additionally, 3D-GS~\cite{3dgs} is notable for its pure explicit representation and differential point-based splatting methods, enabling real-time rendering of novel views. Dynamic3DGS~\cite{dynamic3dgs} models dynamic scenes by tracking the position and variance of each 3D Gaussian at each timestamp $t_i$. An explicit table is utilized to store information about each 3D Gaussian at every timestamp, leading to a linear memory consumption increase, denoted as $O(t\mathcal{N})$, in which $\mathcal{N}$ is num of 3D Gaussians. For long-term scene reconstruction, the storage cost will become non-negligible. The memory complexity of our approach only depends on the number of 3D Gaussians and parameters of Gaussians deformation fields network $\mathcal{F}$, which is denoted as $O(\mathcal{N}+\mathcal{F})$.~\cite{4dgs-2} adds a marginal temporal Gaussian distribution into the origin 3D Gaussians, which uplift 3D Gaussians into 4D. However, it may cause each 3D Gaussian to only focus on their local temporal space. Our approach also models 3D Gaussian motions but with a compact  network, resulting in highly efficient training efficiency and real-time rendering.  


==> sec/3_approachs.tex <==


\section{Method}
\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{fig/coarse2fine.pdf}
   \caption{Illustration of the optimization process. With static 3D Gaussian initialization, our model can learn high-quality 3D Gaussians of the motion part. }
   \label{fig: coarse2fine}
   \vspace{-10pt}
\end{figure}
% framework
    % -->>>>>编码时间的变化,
    % -->>>>>canonical space mapping
    % -->>>>>encode both position and shape deformation
% deformation fields
    % to capture both nearby and far-distance movement, multi-resolution voxel planes are considered.
    % The motion of each point is very direct, so a tiny MLP is strong enough to decode the information.
% optimization
    % two-stage training
    % TV Loss
Sec.~\ref{subsec:4dgs} introduces the overall 4D Gaussian Splatting framework. Then, the Gaussian deformation field is proposed in Sec.~\ref{subsec:filed}. Finally, we describe the optimization process in Sec.~\ref{subsec:optimization}. 

\subsection{4D Gaussian Splatting Framework}
\label{subsec:4dgs}
% Adopting a deformation field to encode 4D information is a common approach in related works~\cite{pumarola2021dnerf,tineuvox}. Given a rendered pixel, a ray $r$ is cast. The sampled points $x$ and timestamp $t$ are fed into an MLP to map into a canonical space and applied with volume rendering~\cite{drebin1988volume}. However, each point on the sample ray may own different velocity variables, which causes heavily different deformation, as shown in Fig.~\ref{fig: splatting-volume}, after applying canonical mapping, the position of each ray is changed. so the volume rendering process may become inaccurate. Meanwhile, differential splatting~\cite{yifan2019differentiablesplatting} creates a relationship among 3D Gaussians on the rendered pixel directly, therefore, each rendered pixel may influenced by different 3D Gaussians every timestamp. The differential splatting is still meaningful. Therefore, we only maintain one set of canonical 3D Gaussians, what we need to do is to employ deformation fields $\mathcal{F}$ to predict each 3D Gaussian's state at a given timestamp $t$.

As shown in Fig.~\ref{fig: pipeline}, given a view matrix $M=[R, T]$, timestamp $t$, our 4D Gaussian splatting framework includes 3D Gaussians $\mathcal{G}$ and Gaussian deformation field network $\mathcal{F}$. Then a novel-view image $\hat{I}$ is rendered by differential splatting~\cite{yifan2019differentiablesplatting} $\mathcal{S}$ following $\hat{I} = \mathcal{S}(M,\mathcal{G}^\prime)$, where $\mathcal{G}^\prime=\Delta\mathcal{G}+\mathcal{G}$.

Specifically, the deformation of 3D Gaussians $\Delta \mathcal{G}$ is introduced by the Gaussian deformation field network $\Delta \mathcal{G} = \mathcal{F}(\mathcal{G}, t)$, in which the spatial-temporal structure encoder $\mathcal{H}$ can encode both the temporal and spatial features of 3D Gaussians $f_d=\mathcal{H}(\mathcal{G}, t)$, and the multi-head Gaussian deformation decoder $\mathcal{D}$ can decode the features and predict each 3D Gaussian's deformation $\Delta \mathcal{G} = \mathcal{D}(f)$, then the deformed 3D Gaussians $\mathcal{G}^\prime$ can be introduced.

% Finally, differential Gaussian splatting~\cite{yifan2019differentiablesplatting} is applied to the deformed 3D Gaussians to render a novel view image.

The rendering process of our 4D Gaussian Splatting is depicted in Fig.~\ref{fig: splatting-volume}~\textcolor{red}{(c)}. Our 4D Gaussian splatting converts the original 3D Gaussians $\mathcal{G}$ into another group of 3D Gaussians $\mathcal{G}^\prime$ given a timestamp $t$, maintaining the effectiveness of the differential splatting as referred in~\cite{yifan2019differentiablesplatting}.

% \begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{fig/voxelgrid.pdf}
%    \caption{Illustration of querying multi-resolution voxel grids.}
%    \label{fig: voxelgrid}
% \end{figure}




\begin{figure*}
   \centering
   \includegraphics[width=1.0\linewidth]{fig/dnerf_result.pdf}
   \caption{Visualization of synthesized datasets compared with other models~\cite{hexplane,kplanes,tineuvox,3dgs,guo2023forwardflowfornvs,msth}. The rendering results of~\cite{kplanes} are displayed with a default green background. We have adopted their rendering settings.}
      \label{fig: dnerf_result}
      \vspace{-10pt}
\end{figure*}

\subsection{Gaussian Deformation Field Network}
\label{subsec:filed}

The network to learn the Gaussian deformation field includes an efficient spatial-temporal structure encoder $\mathcal{H}$ and a Gaussian deformation decoder $\mathcal{D}$ for predicting the deformation of each 3D Gaussian.

\paragraph{Spatial-Temporal Structure Encoder.}

Nearby 3D Gaussians always share similar spatial and temporal information. To model 3D Gaussians' features effectively, we introduce an efficient spatial-temporal structure encoder $\mathcal{H}$ including a multi-resolution HexPlane $R(i,j)$ and a tiny MLP $\phi_d$ inspired by ~\cite{tineuvox,hexplane,kplanes,tensor4d}. While the vanilla 4D neural voxel is memory-consuming, we adopt a 4D K-Planes~\cite{kplanes} module to decompose the 4D neural voxel into 6 planes. All 3D Gaussians in a certain area can be contained in the bounding plane voxels and Gaussian's deformation can also be encoded in nearby temporal voxels.
% To compute the features of 3D Gaussians, bilinear interpolation is employed, which also models the relationship of nearby 3D Gaussians. 

Specifically, the spatial-temporal structure encoder $\mathcal{H}$ contains 6 multi-resolution plane modules $R_l(i,j)$ and a tiny MLP $\phi_d$, \ie $\mathcal{H}(\mathcal{G},t)=\{R_l(i,j), \phi_d | (i,j) \in \{(x,y),(x,z),(y,z),(x,t),(y,t),(z,t)\}, l \in \{1,2\}\}$. The position $\mathcal{X} = (x,y,z)$ is the mean value of 3D Gaussians $\mathcal{G}$. Each voxel module is defined by $R(i,j)\in \mathbb{R}^{h\times l N_i \times l N_j}$, where $h$ stands for the hidden dim of features, $N$ denotes the basic resolution of voxel grid and $l$ equals to the upsampling scale. 
This entails encoding information of the 3D Gaussians within the 6 2D voxel planes while considering temporal information. The formula for computing separate voxel features is as follows:
\begin{equation}
\begin{aligned}
  % f_{voxel} &= \mathcal{F}(\mathcal{X},t)\\
  f_h &= \bigcup_l \prod \text{interp}(R_l(i,j)), \\
    (i,j) &\in \{(x,y),(x,z),(y,z),(x,t),(y,t),(z,t)\}. 
\end{aligned}
\label{formula:feature_position}
\end{equation}
$f_{h} \in \mathbb{R}^{h*l}$ is the feature of neural voxels. `interp' denotes the bilinear interpolation for querying the voxel features located at 4 vertices of the grid. The discussion of the production process is similar to~\cite{kplanes}. Then a tiny MLP $\phi_d$ merges all the features by $f_d = \phi_d(f_h)$.

% In the compact representation of 3D Gaussians, the position $\mathcal{X}$ and time $t$ of these 3D Gaussians play a crucial role in encoding their motion. Besides, as shown in Fig.~\ref{fig: coarse2fine}, during the optimization, the point of Gaussians becomes denser, which means that the covariance of 3D Gaussians is decreasing. Meanwhile, when we introduce additional parameters like covariance values $s$ and $r$ into these 3D Gaussians, it increases the computational demands, leading to a slowdown in both rendering and training speeds. So we conclude that the covariance of Gaussians will become less important during the optimization. Therefore, we omit the 3D Gaussian's rotation and scaling information and focus solely on the position $\mathcal{X}$ and given timestamp $t$. 

\paragraph{Multi-head Gaussian Deformation Decoder.}
\label{subsec:Gaussian Deformation Decoder}

When all the features of 3D Gaussians are encoded, we can compute any desired variable with a multi-head Gaussian deformation decoder $\mathcal{D}=\{\phi_x, \phi_r, \phi_s\}$. Separate MLPs are employed to compute the deformation of position $\Delta \mathcal{X} = \phi_x(f_d)$, rotation $\Delta r= \phi_r(f_d)$, and scaling $\Delta s=\phi_s(f_d)$.
Then, the deformed feature $(\mathcal{X}^\prime,r^\prime,s^\prime)$ can be addressed as:
\begin{align}
    & (\mathcal{X}^\prime, r^\prime, s^\prime) = (\mathcal{X} + \Delta \mathcal{X}, r + \Delta r, s + \Delta s) .
\end{align}
Finally, we obtain the deformed 3D Gaussians $\mathcal{G}^\prime=\{\mathcal{X}^\prime, s^\prime, r^\prime,\sigma,\mathcal{C} \}$.


% \paragraph{Empty Voxel Mask Grid for Multi-cams Setups.}
% In the multi-video setups, dynamic scenes can be modelled by 4D-GS precisely and both the motion part and static part can be divided. Therefore, we proposed a empoty voxel mask $\mathcal{M}$ to split the static 3D Gaussians and dynamic 3D Gaussians explicitly. Speficially, all the deformation value $( \Delta \mathcal{X},\Delta r,\Delta s ) $ computed by Gaussian Deformation Decoder will be multipied by a motion ratio tri-linearly interpolated by the explicit voxel grid $\delta = \mathcal{M}(\mathcal{X})$. The deformation of all the 3D Gaussians will be replaced by:
% \begin{align}
%     & (\mathcal{X}^\prime, r^\prime, s^\prime) = (\mathcal{X} + \Delta \mathcal{X}*\delta, r + \Delta r * \delta, s + \Delta s * \delta) .
% \end{align}
% As is shown in Fig.~\ref{fig: empty_voxel_vis}, multi-cams setups can boost 4D-GS decompose static and dynamic part easily, explicit empoty voxel also guided the optimization of model, which contribute to rendering qualities.

% \begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{fig/voxel_vis.pdf}
%    \caption{Visualization of dynamic scene point clouds and Empty Voxel Mask grid. The colored point stand for non-zero value of the empty voxel mask grid. Note that edged of the scenes only captured by few cameras, which causes failure of modeling.}
%    \label{fig: empty_voxel_vis}
% \end{figure}

    
\subsection{Optimization}
\label{subsec:optimization}



\paragraph{3D Gaussian Initialization.}
\cite{3dgs} shows that 3D Gaussians can be well-trained with structure from motion (SfM)~\cite{schonberger2016structure} points initialization. Similarly, 4D Gaussians should also be fine-tuned in proper 3D Gaussian initialization. We optimize 3D Gaussians at initial 3000 iterations for warm-up and then render images with 3D Gaussians $\hat{I} = \mathcal{S}(M,\mathcal{G})$ instead of 4D Gaussians $\hat{I}=\mathcal{S}(M,\mathcal{G}^\prime)$. The illustration of the optimization process is shown in Fig.~\ref{fig: coarse2fine}.


% Direct optimizing 4D-GS may cause disturbing even failure in both learning the deformation field and 3D Gaussians. So we have to initialize random 3D Gaussians $\mathcal{S}$ in the manually defined bounding box and train the $\mathcal{S}$ only, then 4D Gaussians $\mathcal{G}=\{ \mathcal{S},\mathcal{D},\mathcal{F} \}$ feed activated in the joint optimization process. 



% \begin{algorithm}
%      \caption{Active 3D Gaussians Growing}
%      \label{algorithm: Active 3D Gaussians Growing}
%     \begin{algorithmic}[1]
%      \Require $\mathcal{S}$
%      \Require $N_{down},N_{thres}$
%      \Require $mindis,radii$
%      \Ensure New 3D Gaussians $\mathcal{S}+\mathcal{\hat{S}}$
%      \State  $\mathcal{S}_0 \leftarrow \mathcal{S}$
%      \State  $\mathcal{\hat{S}} \leftarrow \{\}$

%      \While{num of $\mathcal{S}_0 < N_{down}$ }
%         \State $\mathcal{S}_0 \leftarrow $ Downsample($\mathcal{S}_0$)
%      \EndWhile
%      \While{$\hat{S} < N_{thres} $}
%           \ForAll {3D Gaussians $s_i$ in $\mathcal{S}_0$}
%         \State $d$ = SearchNearest($s_i$)
%         \If{ $d>$ $mindis$}
%               \State $\mathcal{\hat{S}} \leftarrow \{\mathcal{\hat{S}}, s_i + radii*random(size=3)\}$ 
%         \EndIf
%         \State $mindis \leftarrow mindis / 2$ 
%         \State $radii \leftarrow radii / 2$ 

        
%      \EndFor
%      \EndWhile

     
%     \end{algorithmic}
% \end{algorithm}


% \paragraph{Active 3D Gaussians Growing.}
% For the unbounded scenes in the feed-forward settings, sfm~\cite{schonberger2016structurefrommotion} cannot reconstruct all the details of the far-distant area. Which cause to fail of optimizing 3DGS and 4DGS. The reason is that splitting \& cloning 3D Gaussians following gradient flow only cannot cover the area which is far from capturing cameras and own less 3D Gaussians provided by sfm. Meanwhile, far-distant 3D Gaussians are always ignored by differential splatting, which lead to the low gradient value and the difficult of 3D Gaussians' growth. 

% To solve the problem, we propose a active 3D Gaussians growing methods to enable 3D Gaussians' growth.
\paragraph{Loss Function.}
Similar to other reconstruction methods~\cite{3dgs,pumarola2021dnerf,tineuvox}, we use the L1 color loss to supervise the training process. A grid-based total-variational loss~\cite{dvgo,tineuvox,hexplane,kplanes} $\mathcal{L}_{tv}$ is also applied.
\begin{equation}
    % \mathcal{L} = \lambda_1(\hat{c} - c)^2 + \lambda_2\mathcal{L}_{ssim}{(\hat{c},c)} + \lambda_3\mathcal{L}_{lpips}{(\hat{c},c)} + \lambda_4  \mathcal{L}_{constraint}.
    \mathcal{L} = \hat{I} - I + \mathcal{L}_{tv}.
\end{equation}
% $\lambda_i$ are hyperparameters can be manually selected before the beginning of training.

==> sec/4_experiments.tex <==






\begin{figure}
   \centering
   \includegraphics[width=0.95\linewidth]{fig/hyper_result.pdf}
    \caption{Visualization of the HyperNeRF~\cite{park2021hypernerf} datasets compared with other methods~\cite{3dgs,park2021hypernerf,tineuvox,guo2023forwardflowfornvs}. `GT' stands for ground truth images.}
      \label{fig:hyper_result}
    \vspace{-20pt}
\end{figure}


\begin{figure}
   \centering
   \includegraphics[width=0.9\linewidth]{fig/ab_nodrdx.pdf}
   \caption{Ablation Study of the rotation and scaling decoder. `ds'  denotes as $\phi_s$ and, `'dr' stands for $\phi_r$.}
      \label{fig:ab_nodrdx}
    \vspace{-10pt}
\end{figure}










\begin{table*} 
\small
\centering
\caption{Quantitative results on the synthesis dataset. The \colorbox{pink}{best} and the \colorbox{yellow}{second best} results are denoted by pink and yellow. The rendering resolution is set to 800$\times$800. ``Time'' in the table stands for training times.}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{l|ccc|c|cc} 
\toprule
Model  & PSNR(dB)↑ & SSIM↑ & LPIPS↓ & Time↓ &  FPS ↑ & Storage (MB)↓  \\
\midrule  
TiNeuVox-B~\cite{tineuvox}  & 32.67 & 0.97 &  0.04 & 28 mins & 1.5 & 48\\ 
KPlanes~\cite{kplanes} & 31.61 & 0.97 &-& 52 mins& 0.97   &418\\ 
HexPlane-Slim~\cite{hexplane} & 31.04 & 0.97 & 0.04&11m 30s& 2.5 &38\\ 
3D-GS~\cite{3dgs} &23.19 & 0.93 & 0.08&10 mins  \cellcolor{yellow}&\cellcolor{pink}170&\cellcolor{pink}10 \\

FFDNeRF~\cite{guo2023forwardflowfornvs}&\cellcolor{yellow}32.68&0.97&0.04&-&$<$ 1&440\\

MSTH~\cite{msth}&31.34&\cellcolor{yellow}0.98&\cellcolor{yellow}0.02&\cellcolor{pink}6 mins&-&-\\
Ours & \cellcolor{pink}34.05&\cellcolor{pink}0.98 &\cellcolor{pink}0.02\cellcolor{pink}& 20 mins&\cellcolor{yellow}82 &\cellcolor{yellow}18 \\
\bottomrule
\end{tabular}  

\label{table_dnerf}
\end{table*}

\begin{table*} 
\centering
\small
\caption{Quantitative results on HyperNeRF's~\cite{park2021hypernerf} vrig dataset. Rendering resolution is set to 960$\times$540.}
\setlength{\tabcolsep}{13pt}
\begin{tabular}{l|cc|c|cc} 
\toprule  
Model  & PSNR(dB)↑ & MS-SSIM↑  & Times↓ &  FPS↑ & Storage(MB)↓\\ 
\midrule  
Nerfies~\cite{park2021nerfies}&22.2&0.803&$\sim$ hours&$<$ 1&-\\
HyperNeRF~\cite{park2021hypernerf}&22.4&0.814&32 hours &$<$ 1&-\\
TiNeuVox-B~\cite{tineuvox}&\cellcolor{yellow}24.3&0.836&\cellcolor{pink}30 mins&1&\cellcolor{pink}48\\
3D-GS~\cite{3dgs}&19.7&0.680&\cellcolor{yellow}40 mins&\cellcolor{pink}55&\cellcolor{yellow}52\\
FFDNeRF~\cite{guo2023forwardflowfornvs}&24.2&\cellcolor{yellow}0.842&-&0.05&440\\
Ours&\cellcolor{pink}25.2&\cellcolor{pink}0.845&1 hour& \cellcolor{yellow}34&61\\
\bottomrule
\end{tabular}  
\label{tab:hypernerf}
\end{table*}


\begin{table*} 
\centering
\caption{Quantitative results on the Neu3D's~\cite{li2022neural} dataset, rendering resolution is set to 1352$\times$1014.}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{l|ccc|c|cc}  
\toprule
Model  & PSNR(dB)↑ & D-SSIM↓ & LPIPS↓ & Time ↓  & FPS↑ & Storage (MB)↓ \\ 
\midrule 
% Neural Volumes  & 22.800 & 0.062 & 0.295 & - & 1352 × 1014 &- &- \\ 
% LLFF & 23.239 & 0.076 & 0.235 & -& 1352 × 1014&-\\ 
% NeRF-T  & 28.449 & 0.023 & 0.100 &- &1352 × 1014 & 0.011&-\\ 
% DyNeRF  & 29.581 & 0.020 & 0.099 & 1344 hours &1352 × 1014&0.011&- \\  
NeRFPlayer~\cite{song2023nerfplayer}  & 30.69 &  0.034  & 0.111  &  6 hours& 0.045&-\\  
HyperReel~\cite{attal2023hyperreel} &31.10&0.036&0.096&9 hours&2.0&360\\
% K-Planes&31.63&0.018&-&108 mins&-&-&
% HexPlane   & 29.470 & 0.018 & 0.078 & 12 hours &1024 × 768&- &-\\ 
% Ours-batch1*& \textbf{31.15} & 0.9388 &0.1375 & 40 mins  & 30 & 150 M\\
% MixVoxels-L1& 30.80 &0.960&  -  &    1.3 hours&  -&-&-&\\
HexPlane-all*~\cite{hexplane} & 31.70 & \cellcolor{pink}0.014 & 0.075 & 12 hours &0.2&250\\ 
KPlanes~\cite{kplanes}& 31.63& -   &  - &   1.8 hours  &0.3&309\\
Im4D~\cite{lin2023im4d}&\cellcolor{pink}32.58&-&0.208&\cellcolor{yellow}28 mins&$\sim$5&\cellcolor{yellow}93\\
MSTH~\cite{msth}&\cellcolor{yellow}32.37&\cellcolor{yellow}0.015&\cellcolor{yellow}0.056&\cellcolor{pink}20 mins & \cellcolor{yellow}2(15$^\ddag$)&135\\
Ours& 31.15 & 0.016 &\cellcolor{pink}0.049 & 40 mins  &\cellcolor{pink}30 & \cellcolor{pink}90\\
\hline  
\end{tabular}  

 \begin{tablenotes}
        \footnotesize
        \item[*] *: The metrics of the model are tested without ``coffee martini'' and resolution is set to 1024$\times$768. 
        \item [$^\ddag$] $^\ddag$: The FPS is tested with fixed-view rendering.
        \end{tablenotes}\label{tab:dynerf}

\end{table*}

\begin{table*} 
\centering


\caption{Ablation studies on synthetic datasets using our proposed methods.}

% \resizebox{\linewidth}{!}{
% \setlength{\tabcolsep}{0pt} % 缩小列之间的间距

\begin{tabular}{l|ccc|c|ccc} 
\toprule
Model  & PSNR(dB)↑ & SSIM↑ & LPIPS↓ & Time↓ &FPS↑& Storage (MB)↓&\\
\midrule 
Ours w/o HexPlane $R_l(i,j)$ & 27.05 & 0.95 & 0.05& \cellcolor{pink}10 mins &\cellcolor{pink}140 &\cellcolor{pink}12 \\ 
Ours w/o initialization  &31.91 & 0.97 & 0.03&\cellcolor{yellow}19 mins& 79&18 \\ 
Ours w/o $\phi_x$ &26.67&0.95&0.07&20 mins&82&17\\
Ours w/o $\phi_r$ &33.08\cellcolor{yellow}&\cellcolor{yellow}0.98&\cellcolor{yellow}0.03&20 mins&83\cellcolor{yellow}&\cellcolor{yellow}17\\
Ours w/o $\phi_s$ &33.02&0.98&0.03&20 mins&82&17\\ 
Ours & \cellcolor{pink}34.05&\cellcolor{pink}0.98 &\cellcolor{pink}0.02&20 mins&82 &18 \\

\bottomrule
\end{tabular}  
% }
\label{table_ab}
\vspace{-10pt}
\end{table*}


\section{Experiment}

In this section, we mainly introduce the hyperparameters and datasets of our settings in Sec.~\ref{Experimental Setting} and the results between different datasets will be compared with \cite{tineuvox,msth,wang2023mixedvoxels,lin2023im4d,attal2023hyperreel,hexplane,kplanes,3dgs,song2023nerfplayer} in Sec.~\ref{subsec:result}. Then, ablation studies are proposed to prove the effectiveness of our approaches in Sec.~\ref{subsec:ablation study} and more discussion about 4D-GS in Sec.~\ref{subsec:discussions}. Finally, we discuss the limitation of our proposed 4D-GS in Sec.~\ref{Subsec:limitation}.
\subsection{Experimental Settings}
\label{Experimental Setting}
Our implementation is primarily based on the PyTorch~\cite{pytorch} framework and tested in a single RTX 3090 GPU, and we've fine-tuned our optimization parameters by the configuration outlined in the 3D-GS~\cite{3dgs}. More hyperparameters will be shown in the appendix.
% Notably, we have configured the intervals for point cloud pruning to be set at 8000, and the total training iterations decrease to 20000. Additionally, we have established the voxel plane resolution as $[64,64]$, integrating multi-resolution upsampling at levels  $L = \{2,4,8\}$. Following a similar approach to that elucidated in ~\cite{fridovich2023k}, each plane is endowed with hidden features set to a dimension of 32.

% Moreover, the default setting for the hidden layer of the MLP decoder is 64, and the learning rate is initially set at 1.6e-4, gradually decreasing exponentially to 1.6e-6 by the end of the training process. The learning rate for the voxel grid is initialized at 1.6e-3 and exponentially decays to 1.6e-5.

\paragraph{Synthetic Dataset.}We primarily assess the performance of our model using synthetic datasets, as introduced by D-NeRF~\cite{pumarola2021dnerf}. These datasets are designed for monocular settings, although it's worth noting that the camera poses for each timestamp are close to randomly generated. Each scene within these datasets contains dynamic frames, ranging from 50 to 200 in number.
\paragraph{Real-world Datasets.} We utilize datasets provided by HyperNeRF~\cite{park2021hypernerf} and Neu3D's~\cite{li2022neural} as benchmark datasets to evaluate the performance of our model in real-world scenarios. The Nerfies dataset is captured using one or two cameras, following straightforward camera motion, while the Neu3D's dataset is captured using 15 to 20 static cameras, involving extended periods and intricate camera motions. We use the points computed by SfM~\cite{schonberger2016structure} from the first frame of each video in Neu3D's dataset and 200 frames randomly selected in HyperNeRF's.
% \subsection{Metrics}
% \begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{fig/ab_coarse2fine.pdf}
%    \caption{Ablation Study of two stages training. Without static point cloud initialization, Gaussians may go into local minimum and suffer from a worse quality.}
%    \label{fig: ab_coarse2fine}
% \end{figure}
% \begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{fig/ab_tv.pdf}
%    \caption{Ablation Study of total variation loss mentioned in ~\cite{kplanes}, with TV loss adopted in voxel grid, the training process will become smoother and enjoy better results.}
%    \label{fig: ab_tv}
% \end{figure}
\subsection{Results}
\label{subsec:result}
We primarily assess our experimental results using various metrics, encompassing peak-signal-to-noise ratio (PSNR), perceptual quality measure LPIPS~\cite{lpips}, structural similarity index (SSIM)~\cite{ssim} and its extensions including structural dissimilarity index measure (DSSIM), multiscale structural similarity index (MS-SSIM), FPS, training times and Storage. 
% Notably, our approach stands out with its relatively swift training pace and exceptionally rapid rendering speed and can handle both monocular and multi-cams setups, achieving over 80 FPS at a resolution of 800$\times$800.

To assess the quality of novel view synthesis, we conducted benchmarking against several state-of-the-art methods in the field, including ~\cite{tineuvox,hexplane,kplanes,msth,3dgs}. The results are summarized in Tab.~\ref{table_dnerf}. While current dynamic hybrid representations can produce high-quality results, they often come with the drawback of rendering speed. The lack of modeling dynamic motion part makes~\cite{3dgs} fail to reconstruct dynamic scenes. In contrast, our method enjoys both the highest rendering quality within the synthesis dataset and exceptionally fast rendering speeds while keeping extremely low storage consumption and convergence time.

Additionally, the results obtained from real-world datasets are presented in Tab.~\ref{tab:hypernerf} and Tab.~\ref{tab:dynerf}. It becomes apparent that some NeRFs~\cite{song2023nerfplayer,attal2023hyperreel,hexplane} suffer from slow convergence speed, and the other grid-based NeRF methods~\cite{tineuvox,hexplane,msth,kplanes} encounter difficulties when attempting to capture intricate object details. In stark contrast, our methods research comparable rendering quality, fast convergence, and excel in free-view rendering speed in indoor cases. Though~\cite{lin2023im4d} addresses the high quality in comparison to ours, the need for multi-cam setups makes it hard to model monocular scenes and other methods also limit free-view rendering speed and storage.
\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{fig/grid_vis.pdf}
   \caption{Visualization of HexPlane voxel grids. (a) are the rendered images. (b) are the parameters of spatial voxel grids, which implies the feature of 3D Gaussians are encoded in explicit grids. (c) are the temporal features of the grids, each column stands for spatial features in the timestamps.}
   \label{fig: vis_voxelgrid}
\end{figure}

\subsection{Ablation Study}
\label{subsec:ablation study}
\paragraph{Spatial-Temporal Structure Encoder.}
The explicit HexPlane encoder $R_l(i,j)$ possesses the capacity to retain 3D Gaussians' spatial and temporal information, which can reduce storage consumption in comparison with purely explicit methods~\cite{dynamic3dgs}. Discarding this module, we observe that using only a shallow MLP $\phi_d$ falls short in modeling complex deformations across various settings. Tab.~\ref{table_ab} demonstrates that, while the model incurs minimal memory costs, it does come at the expense of rendering quality. 
% \paragraph{Model Capacity.}

% Undoubtedly, expanding the model's size, be it through increased voxel plane resolutions or deeper MLP decoders, can significantly elevate rendering quality. However, this enhancement invariably carries the trade-off of diminished rendering speed, owing to the heightened computational demands imposed by larger models. Tab.~\ref{table_ab} provides concrete evidence of this trade-off. When we augment the hidden layer of the MLP to a size of 256, we observe a noteworthy improvement in rendering quality, translating to an approximate gain of 0.25 dB. 

\vspace{-3pt}
\paragraph{Gaussian Deformation Decoder.}
Our proposed Gaussian deformation decoder $\mathcal{D}$ decodes the features from the spatial-temporal structure encoder $\mathcal{H}$. All the changes in 3D Gaussians can be explained by separate MLPs $\{\phi_x,\phi_r,\phi_s\}$. As is shown in Tab.~\ref{table_ab}, 4D Gaussians cannot fit dynamic scenes well without modeling 3D Gaussian motion. Meanwhile, the movement of human body joints is typically manifested as stretching and twisting of surface details in a macroscopic view. If one aims to accurately model these movements, the size and shape of 3D Gaussians should also be adjusted accordingly. Otherwise, there may be underfitting of details during excessive stretching, or an inability to correctly simulate the movement of objects at a microscopic level.  Fig.~\ref{fig:ab_nodrdx} also demonstrates that shape deformation of 3D Gaussians is important in recovering details.
\vspace{-3pt}
\paragraph{3D Gaussian Initialization.}
In some cases without SfM~\cite{schonberger2016structure} points initialization, training 4D-GS directly may cause difficulty in convergence. Optimizing 3D Gaussians for warm-up enjoys: (a) making some 3D Gaussians stay in the dynamic part, which releases the pressure of large deformation learning by 4D Gaussians as shown in Fig.~\ref{fig: coarse2fine}. (b) learning proper 3D Gaussians $\mathcal{G}$ and suggesting deformation fields paying more attention to the dynamic part like Fig.~\ref{fig: vis_voxelgrid}\textcolor{red} {(c)}. 
(c) avoiding numeric errors in optimizing the Gaussian deformation network $\mathcal{F}$ and keeping the training process stable. Tab.~\ref{table_ab} also shows that if we train our model without the warm-up coarse stage, the rendering quality will suffer.
\subsection{Discussions}\label{subsec:discussions}
\vspace{-3pt}
\paragraph{Analysis of Multi-resolution HexPlane Gaussian Encoder.}The visualization of features in our multi-resolution HexPlane $R_l(i,j)$ is depicted in Fig.~\ref{fig: vis_voxelgrid}. As an explicit module, all the 3D Gaussians features can be easily optimized in individual voxel planes. It can be observed in Fig.~\ref{fig: vis_voxelgrid} \textcolor{red}{(b)} that the voxel plane even shows a similar shape to the rendered image, such as edges. Meanwhile, the temporal features also stay in motion areas in the Fig.~\ref{fig: vis_voxelgrid} \textcolor{red}{(c)}. Such an explicit representation boosts the speed of training and rendering quality of our 4D Gaussians.


\vspace{-3pt}
\begin{figure}
   \centering
   \includegraphics[width=0.9\linewidth]{fig/track_point.pdf}
   \caption{Visualization of tracking with 3D Gaussians. Each line in the figure of second rows stands for trajectories of 3D Gaussians}
      \label{fig:point_track}
\end{figure}

\paragraph{Tracking with 3D Gaussians.}Tracking in 3D is also a important task.~\cite{guo2023forwardflowfornvs} also shows tracking objects' motion in 3D. Different from dynamic3DGS~\cite{dynamic3dgs}, our methods even can present tracking objects in monocular settings with pretty low storage \ie 10MB in 3D Gaussians $\mathcal{G}$ and 8 MB in Gaussian deformation field network $\mathcal{F}$. Fig.~\ref{fig:point_track} shows the 3D Gaussian's deformation at certain timestamps.

\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{fig/editing.pdf}
   \caption{Visualization of composition with 4D Gaussians.}
   \label{fig: editing}
   \vspace{-10pt}
\end{figure}
\vspace{-3pt}

\paragraph{Composition with 4D Gaussians.}Similar to dynamic3DGS~\cite{dynamic3dgs}, our proposed methods can also propose editing in 4D Gaussians in Fig.~\ref{fig: editing}. Thanks to the explicit representation of 3D Gaussians, all the trained models can predict deformed 3D Gaussians in the same space following $\mathcal{G}^\prime=\{ \mathcal{G}_1^\prime,\mathcal{G}_2^\prime,...,\mathcal{G}_n^\prime\}$ and differential rendering~\cite{yifan2019differentiablesplatting} can project all the point clouds into viewpoints by $\hat{I} = \mathcal{S}(M,\mathcal{G}^\prime)$.
\begin{figure}
   \centering
   % \vspace{-1pt}
   \includegraphics[width=\linewidth]{fig/point_fps.pdf}
   \caption{Visualization of the relationship between rendering speed and numbers of 3D Gaussians in the rendered screens. All the tests are finished in the synthesis dataset.}
    \label{fig:point_fps}
    \vspace{-15pt}
\end{figure}
\vspace{-3pt}
\paragraph{Analysis of Rendering Speed.} As is shown in Fig.~\ref{fig:point_fps}, we also test the relationship between points in the rendered screen and rendering speed at the resolution of 800$\times$800. We found that if the rendered points are lower than 30000, the rendering speed can be up to 90. The config of Gaussian deformation fields are discussed in the appendix. To achieve render-time rendering speed, we should strike a balance among all the rendering resolutions, 4D Gaussians representation including numbers of 3D Gaussians, and the capacity of the Gaussian deformation field network and any other hardware constraints.

% \paragraph{Empty Voxel Mask Grid.}
% For mutli-cams setups, the weight provided by empty voxel mask grid can correct the deformation fields' output, add the mask grid would contribute to PSNR by 0.4 dB. Fig.~\ref{fig: ab_emptyvoxel} shows the difference between training with empoty voxel mask grid or optimizing without it.
% In datasets such as D-NeRF~\cite{pumarola2021dnerf} and DyNeRF~\cite{li2022neural}, there is no prior point cloud information available for initializing 3D Gaussians. Consequently, training the model to learn both 3D Gaussians and deformation fields becomes considerably more challenging compared to static scenes. To address this issue, we adopt the strategy of optimizing 3D Gaussians exclusively, allowing the model to establish a suitable initialization for learning the motion fields. As illustrated in Fig.~\ref{fig: ab_coarse2fine}, through a brief static training stage of just $N=3000$ iterations (lasting no more than 2 minutes), we observe a notable improvement of approximately 1.5 dB in the PSNR of the scene.

% Conversely, eliminating the 8x upsampling resolution negatively impacts the results, demonstrating its critical role in maintaining rendering quality.

% \paragraph{Fast Training.}Conversely, stopping the model's training at iteration 7k can still yield relatively good results, this approach has the potential to train a faster coarse model. The results of fast training are also displayed in Tab.~\ref{table_ab}.

% \paragraph{Image-based Loss.}
% We owe a significant portion of our progress to the splatting algorithm. In every training stage, an image is generated by the model based on the provided training camera pose. This allows us to apply LPIPS-based~\cite{lpips} Loss and SSIM-based~\cite{ssim} Loss during the training process. However, it's essential to acknowledge that this inclusion does slow down the training speed by over 2 times, potentially impeding real-time rendering. It may be because optimizing the motion part is a hard and complex process. Adding image-based loss may trigger worse cases. As a result, during the training stage, we have chosen to decelerate this process to ensure more efficient model training.


% \begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{fig/dynerf_result.pdf}
%    \caption{Visualization of DyNeRF's rendering results through our model, as referenced in \cite{li2022neural}.}
%       \label{fig: dynerf_result}

% \end{figure}
\subsection{Limitations}
\label{Subsec:limitation}
Though 4D-GS can indeed attain rapid convergence and yield real-time rendering outcomes in many scenarios, there are a few key challenges to address. First, large motions, the absence of background points, and the unprecise camera pose cause the struggle of optimizing 4D Gaussians. What is more, it is still challenging to 4D-GS also cannot split the joint motion of static and dynamic Gaussiansparts under the monocular settings without any additional supervision. Finally, a more compact algorithm needs to be designed to handle urban-scale reconstruction due to the heavy querying of Gaussian deformation fields by huge numbers of 3D Gaussians. 

\section{Conclusion}
This paper proposes 4D Gaussian splatting to achieve real-time dynamic scene rendering. An efficient deformation field network is constructed to accurately model Gaussian motions and shape deformations, where adjacent Gaussians are connected via a spatial-temporal structure encoder. Connections between Gaussians lead to more complete deformed geometry, effectively avoiding avulsion. Our 4D Gaussians can not only model dynamic scenes but also have the potential for 4D objective tracking and editing.
% an advanced dynamic scene reconstruction algorithm capable of delivering high-quality results while enabling real-time rendering. While Gaussian representation proves effective for achieving high-quality rendering results in indoor environments, it's important to note that the omission of background point modeling remains an area of interest and warrants further investigation.










